CalibForge: Adversarial Solver Calibration for Scaling Learnable Terminal Tasks

Training terminal agents requires executable and verifiable tasks that are not merely solvable, but appropriately challenging for learning. Executable validation establishes feasibility, yet does not reveal how a task behaves relative to a given solver setting. In this paper, we present CalibForge, an autonomous terminal-task synthesis system that uses verified solver behavior to revise candidate tasks through adversarial solver calibration. Multi-solver calibration targets disagreement within a heterogeneous solver pool, whereas contrastive solver calibration targets a designated strong-pass/weak-fail relation; both operationalize a solver-relative learnable zone anchored in demonstrated solvability. Using CalibForge, we construct 5,431 calibrated terminal tasks. Our ablations show that both strategies yield more effective supervision than authoring and validation alone or ordinary single-solver feedback. Models trained on the full collection achieve 31.84% and 47.57% on Terminal-Bench 2.1. The largest improvements over the corresponding base model reach 23.97 percentage points on Terminal-Bench 2.1, 26.54 points on SWE-bench Pro, and 30.04 points on Doc2Repo. Together, these results support solver-relative learnability as a practical target for constructing effective and transferable agent training data.

==> section/prompts/calibforge_eval_system_prompt.tex <==
You are a capable code and command-line agent operating in a Linux runtime environment. Complete the user's technical task by inspecting the environment, editing files, running commands, and verifying the result. Use the available tools directly whenever an action is needed.

<WORKFLOW>
1. Read the task carefully and identify the concrete deliverable, required output format, exact paths, field names, variable names, version constraints, and any named interfaces, scripts, files, or services. Treat these details as hard requirements.
2. Survey the environment before changing it. Check the working directory and nearby resources, but do not assume all relevant files are under the initial directory.
3. Prefer existing project workflows and task-provided interfaces over building local substitutes. If a CLI, script, API, or data format is mentioned, inspect its help, documentation, source, or sample data before using it.
4. Pay attention to implicit constraints in the task wording, especially constraints about exact outputs, allowed files, dependency versions, or how simple the requested solution should be.
5. Make focused changes that solve the task. Modify intended files directly instead of creating alternate copies with suffixes such as _fixed, _new, or _test.
6. Keep deliverable directories clean. Temporary scripts, downloaded files, build outputs, compiled binaries, caches, and exploratory artifacts should stay outside the final deliverable location unless the task explicitly asks for them.
7. Verify the result with task-relevant commands whenever possible. If full verification is expensive or unavailable, run targeted smoke checks that exercise the requested behavior.
8. Finish only after the environment is in the final state needed for grading.
</WORKFLOW>

<TOOL_USE>
Use the bash tool for shell commands, builds, package installation, data processing, service checks, and running verification commands. Use the file editor tool for precise text-file inspection and edits. Prefer absolute paths for file operations.

For text edits, view enough context first and ensure replacements are exact and unique. If several edits to one file are needed, batch them when practical. For multi-line code or structured text, prefer the file editor tool over fragile shell quoting; if you generate files with shell commands, read them back before running them.

Do not add explanatory documentation or extra artifacts unless the task asks for them or they are required by the solution.
</TOOL_USE>

<LONG_RUNNING_WORK>
Some tasks require slow downloads, dependency installation, compilation, model loading, or large data processing. For commands that may take longer than the default command timeout, pass an appropriate timeout value to the bash tool. If a long command times out or produces partial logs, inspect the logs, adjust the approach, and retry with a clearer command, a longer timeout, or a background process with log polling.

When dependencies are missing, first look for existing project files such as requirements.txt, pyproject.toml, package.json, Cargo.toml, Makefile, or README instructions. Prefer the repository's declared setup path over ad-hoc package installs, but install missing dependencies when necessary to complete the task.

Network downloads may be slow or partially blocked. For GitHub, Hugging Face, PyPI, apt, video sites, and large artifacts, first identify whether the issue is speed, availability, permission, rate limiting, or anti-bot behavior. For slow downloads, try reliable mirrors, resumable commands, or smaller range checks, then verify the downloaded file's size and format. For video-site or anti-bot failures, look for legitimate mirrors, archives, or alternate sources before relying on an approximation.
</LONG_RUNNING_WORK>

<VERIFICATION>
Do not mark the task complete just because a file was created, a command started, or an import succeeded once. Check the resulting files, imports, command output, tests, service behavior, or structured data that matter for the task. For JSON, CSV, databases, archives, compressed files, or generated reports, load or preview the artifact with an appropriate tool and confirm the schema and contents match the requirement.

If a check fails, use the failure message to continue debugging instead of finishing. If the same approach fails repeatedly, inspect the relevant files, logs, or help output and switch to a different method rather than retrying blindly.

When running provided checks or tests, confirm that the command you ran is the intended entry point. Empty output or a zero exit code is not enough if the task requires a specific file, exact one-line answer, schema, version, or absence of extra files.
</VERIFICATION>

<SAFETY_AND_SCOPE>
Work only on changes needed for the task. Avoid destructive operations unless they are clearly required. Do not rely on hidden grader behavior or hard-code answers for a specific verifier; solve the stated task in the environment. The user will not provide interactive clarification during the run, so make reasonable assumptions and keep working toward a verified final state.
</SAFETY_AND_SCOPE>

When the task is complete, call the finish tool. Do not finish merely by saying the task is done in text.

==> section/prompts/calibforge_eval_user_prompt.tex <==
Task:
{instruction}

Working directory: {workdir}

Complete the task in the current runtime environment. The final state of this environment will be evaluated after you call finish.

==> section/prompts/cross_no_search_user_prompt.tex <==
<uploaded\_files>
{workspace\_dir}
</uploaded\_files>

I've uploaded a python code repository in the directory {workspace\_dir}. Consider the following issue description:

<issue\_description>
{problem\_statement}
</issue\_description>

Can you help me implement the necessary changes to the repository so that the requirements specified in the <issue\_description> are met?
I've already taken care of all changes to any of the test files described in the <issue\_description>. This means you DON'T have to modify the testing logic or any of the tests in any way!
Your task is to make the minimal changes to non-test files in the {workspace\_dir} directory to ensure the <issue\_description> is satisfied.

Follow these phases to resolve the issue:

Phase 1. READING: read the problem and reword it in clearer terms
   1.1 If there are code or config snippets. Express in words any best practices or conventions in them.
   1.2 Highlight message errors, method names, variables, file names, stack traces, and technical details.
   1.3 Explain the problem in clear terms.
   1.4 Enumerate the steps to reproduce the problem.
   1.5 Highlight any best practices to take into account when testing and fixing the issue

Phase 2. RUNNING: install and run the tests on the repository
   2.1 Follow the readme
   2.2 Install the environment and anything needed
   2.3 Iterate and figure out how to run the tests

Phase 3. EXPLORATION: find the files that are related to the problem and possible solutions
   3.1 Use `grep` to search for relevant methods, classes, keywords and error messages.
   3.2 Identify all files related to the problem statement.
   3.3 Propose the methods and files to fix the issue and explain why.
   3.4 From the possible file locations, select the most likely location to fix the issue.

Phase 4. TEST CREATION: before implementing any fix, create a script to reproduce and verify the issue.
   4.1 Look at existing test files in the repository to understand the test format/structure.
   4.2 Create a minimal reproduction script that reproduces the located issue.
   4.3 Run the reproduction script to confirm you are reproducing the issue.
   4.4 Adjust the reproduction script as necessary.

Phase 5. FIX ANALYSIS: state clearly the problem and how to fix it
   5.1 State clearly what the problem is.
   5.2 State clearly where the problem is located.
   5.3 State clearly how the test reproduces the issue.
   5.4 State clearly the best practices to take into account in the fix.
   5.5 State clearly how to fix the problem.

Phase 6. FIX IMPLEMENTATION: Edit the source code to implement your chosen solution.
   6.1 Make minimal, focused changes to fix the issue.

Phase 7. VERIFICATION: Test your implementation thoroughly.
   7.1 Run your reproduction script to verify the fix works.
   7.2 Add edge cases to your test script to ensure comprehensive coverage.
   7.3 Run existing tests related to the modified code to ensure you haven't broken anything.

8. FINAL REVIEW: Carefully re-read the problem description and compare your changes with the base commit {base\_commit}.
   8.1 Ensure you've fully addressed all requirements.
   8.2 Run any tests in the repository related to:
     8.2.1 The issue you are fixing
     8.2.2 The files you modified
     8.2.3 The functions you changed
   8.3 If any tests fail, revise your implementation until all tests pass

Be thorough in your exploration, testing, and analysis. It's fine if your thinking process is lengthy - quality and completeness are more important than brevity.

==> section/prompts/cross_problem_statement.tex <==
# Server ignores `host` argument in `start()` and `TRAME_DEFAULT_HOST` environment variable

## Description
We are encountering an issue where the `host` parameter passed to `trame_server.Server.start()` is ignored, causing the server to always bind to `localhost` (127.0.0.1). This prevents external connections and is blocking downstream integrations that require binding to specific interfaces (e.g., `0.0.0.0` for containerized environments), such as the ongoing work in PyVista (see [pyvista/pyvista#3385](https://github.com/pyvista/pyvista/pull/3385)).

The server persists with the CLI default (`localhost`) even when an explicit override is provided in Python. Furthermore, the `TRAME_DEFAULT_HOST` environment variable, which is expected to define the host when no argument is provided, is currently not respected.

## Steps to Reproduce
The following script attempts to bind the server to `0.0.0.0`, but the server continues to listen on `127.0.0.1`:

```python
import os
from trame_server import Server

# Scenario 1: Attempt to start server on all interfaces via argument
# Expected: Binds to 0.0.0.0
# Actual: Binds to 127.0.0.1
print("--- Testing host argument ---")
server = Server()
try:
    # This host argument is currently ignored
    server.start(port=8080, host='0.0.0.0', open_browser=False)
except Exception as e:
    print(f"Error: {e}")
finally:
    server.stop()

# Scenario 2: Attempt using environment variable
# Expected: Binds to 0.0.0.0
# Actual: Binds to 127.0.0.1 (default)
print("\n--- Testing environment variable ---")
os.environ['TRAME_DEFAULT_HOST'] = '0.0.0.0'
server2 = Server()
try:
    server2.start(port=8081, open_browser=False)
except Exception as e:
    print(f"Error: {e}")
finally:
    server2.stop()
```

## Expected Behavior
1.  **Argument Priority:** When `server.start(host='0.0.0.0')` is called, the server should respect the `host` argument and bind to that address.
2.  **Environment Variable:** If no `host` argument is provided to `start()`, the server should use the value of `TRAME_DEFAULT_HOST` if it is set.

==> section/prompts/cross_search_user_prompt.tex <==
<uploaded\_files>
{workspace\_dir}
</uploaded\_files>

I've uploaded a python code repository in the directory {workspace\_dir}. Consider the following issue description:

<issue\_description>
{problem\_statement}
</issue\_description>

Can you help me implement the necessary changes to the repository so that the requirements specified in the <issue\_description> are met?
I've already taken care of all changes to any of the test files described in the <issue\_description>. This means you DON'T have to modify the testing logic or any of the tests in any way!
Your task is to make the minimal changes to non-test files in the {workspace\_dir} directory to ensure the <issue\_description> is satisfied.

Follow these phases to resolve the issue:

Phase 1. READING: read the problem and reword it in clearer terms
   1.1 If there are code or config snippets. Express in words any best practices or conventions in them.
   1.2 Highlight message errors, method names, variables, file names, stack traces, and technical details.
   1.3 Explain the problem in clear terms.
   1.4 Enumerate the steps to reproduce the problem.
   1.5 Highlight any best practices to take into account when testing and fixing the issue.
   1.6 Identify any external URLs, referenced issues in other repositories, or mentions of external library updates in the <issue\_description>. List these clearly as targets for the search phase.

Phase 2. RUNNING: install and run the tests on the repository
   2.1 Follow the readme
   2.2 Install the environment and anything needed
   2.3 Iterate and figure out how to run the tests

Phase 3. EXPLORATION: find the files that are related to the problem and possible solutions
   3.1 Use `grep` to search for relevant methods, classes, keywords and error messages.
   3.2 Identify all files related to the problem statement.
   3.3 Propose the methods and files to fix the issue and explain why.
   3.4 From the possible file locations, select the most likely location to fix the issue.
   3.5 You can use the **Search Tool** to retrieve the associated URL in the problem statement or other useful information. 
   3.6 **Attention**:
       - **MANDATORY Deep Reading**: If a search result looks promising, you **MUST** use the **LinkSummary** tool to fetch and read the actual page content. Treat search snippets merely as relevance indicators. Snippets are often incomplete or outdated. **Never write code based solely on search snippets.**

Phase 4. TEST CREATION: before implementing any fix, create a script to reproduce and verify the issue.
   4.1 Look at existing test files in the repository to understand the test format/structure.
   4.2 Create a minimal reproduction script that reproduces the located issue.
   4.3 Run the reproduction script to confirm you are reproducing the issue.
   4.4 Adjust the reproduction script as necessary.

Phase 5. FIX ANALYSIS: state clearly the problem and how to fix it
   5.1 State clearly what the problem is, specifically citing any external specifications or dependency changes found during the search phase if relevant.
   5.2 State clearly where the problem is located.
   5.3 State clearly how the test reproduces the issue.
   5.4 State clearly the best practices to take into account in the fix.
   5.5 State clearly how to fix the problem.

Phase 6. FIX IMPLEMENTATION: Edit the source code to implement your chosen solution.
   6.1 Make minimal, focused changes to fix the issue.

Phase 7. VERIFICATION: Test your implementation thoroughly.
   7.1 Run your reproduction script to verify the fix works.
   7.2 Add edge cases to your test script to ensure comprehensive coverage.
   7.3 Run existing tests related to the modified code to ensure you haven't broken anything.

8. FINAL REVIEW: Carefully re-read the problem description and compare your changes with the base commit {base\_commit}.
   8.1 Ensure you've fully addressed all requirements.
   8.2 Run any tests in the repository related to:
     8.2.1 The issue you are fixing
     8.2.2 The files you modified
     8.2.3 The functions you changed
   8.3 If any tests fail, revise your implementation until all tests pass

Be thorough in your exploration, testing, and reasoning. It's fine if your thinking process is lengthy - quality and completeness are more important than brevity.

==> section/prompts/doc2repo_no_search_user_prompt.tex <==
I need you to implement a software repository from scratch based on a strict architectural specification.

### 1. Context & Environment
* **Workspace Directory**: `{workspace_dir}`
* **Current File Structure**:
```text
{workspace_tree}
```
* **Installation Status**: The `target_repo` package is already installed in editable mode (`pip install -e .`). Any changes you make inside the `target_repo/` directory will be immediately reflected in the environment.

### 2. Environment & Dependency Management
The repository will be installed and evaluated using `pip install -e .`. You must manage dependencies strictly via `setup.py`.

<CURRENT_ENVIRONMENT>
The following packages are **ALREADY INSTALLED** in the environment. You can use them directly without reinstalling:
```text
{installed_packages}
```
*(Note: Do not assume any other packages exist unless listed above.)*
</CURRENT_ENVIRONMENT>

<DEPENDENCY_RULES>
1. **Setup.py is King**: You MUST list all necessary runtime dependencies in `setup.py`.
2. **Avoid Redundancy**: If a package is already in **<CURRENT_ENVIRONMENT>**, do **NOT** add it to `setup.py` unless you absolutely need a different version than the one installed. This prevents network timeouts and conflicts in the evaluation environment.
3. **Pin New Dependencies**: If you need a package that is **NOT** in the list above, you **MUST** add it to `setup.py` and **explicitly pin the version**.
4. **Ignore requirements.txt**: Do not create or update `requirements.txt`. Only modify `setup.py`.
</DEPENDENCY_RULES>

### 3. The Specification (`repo_document.md`)
This document is the **Absolute Authority** for the **Architecture, Public API, and Logic**. You must implement the repository exactly as described here.
```markdown
{REPO_DOCUMENT}
```

---

### 4. Task Instructions

**Phase 1: Analysis & Research (Critical Discipline)**
* **Analyze the Spec**: Read `repo_document.md` to deduce the required directory structure and class hierarchy based strictly on the **Import Paths** defined in the document.
* **Check Dependencies**: Compare spec requirements against <CURRENT_ENVIRONMENT>. Decide which ones need to be added to `setup.py` and which ones are already present.

**Phase 2: Implementation**
* Implement the **Public API** and **Core Logic** described in the document inside the `target_repo/` directory.
* **Strict Constraints**:
    * Function signatures (arguments, types, return values) MUST match the document exactly.
    * Ensure all imports use relative imports (e.g., `from . import utils`) or absolute imports starting with `target_repo`.
* **Internal Implementation Flexibility**:
    * The document lists the **Core Public API**. You are encouraged to create necessary **private helper functions**, **internal constants**, or **utility classes** to support the logic.
    * **Guidelines**:
        * Keep internal helpers private (prefix with `_`) where appropriate.
        * You may create new utility files inside the `target_repo/` directory if the logic requires it, but **do not abuse this**—keep the structure clean and logical.
        * Do NOT change the signature of the documented Public APIs.

**Phase 3: Verification (Self-Correction)**
* Since this is a clean-room implementation, **NO existing tests are provided**.
* You are responsible for verifying your own code:
    * Create a standalone script (e.g., `verify_implementation.py`) to import your new classes/functions and assert they behave as documented.
    * OR write simple `pytest` cases to check critical logic.
* **Goal**: Ensure your implementation runs without errors and matches the spec before you finish.

**Phase 4: Submission**
* Once you are confident:
    1. Delete any temporary verification scripts (`verify_implementation.py`) to keep the repo clean.
    2. Ensure `setup.py` is configured correctly according to <DEPENDENCY_RULES>.
    3. Submit your work using the "finish" tool.

==> section/prompts/doc2repo_problem_statement.tex <==
# Specification: target_repo

## 1. Overview
The `target_repo` library is a unified document processing tool designed to convert various document formats (PDF, Office files, Images, HTML, etc.) into clean Markdown. It emphasizes high-fidelity conversion by preserving layout, tables, and extracting images. A key feature is its integration with AI-powered OCR (specifically OpenAI's Vision API and Tesseract) to handle scanned documents and complex layouts that traditional extractors miss.

The library provides a simple, unified API for processing single files or batch-processing entire directories. It abstracts away the complexity of handling different file formats, providing a consistent `ProcessedDocument` output containing the content, metadata, and extracted assets.

## 2. API Reference

### Component: `UnifiedDocumentLoader`

**Import Path:**
`from target_repo import UnifiedDocumentLoader`

**Signature:**
```python
class UnifiedDocumentLoader:
    def __init__(
        self,
        ocr_provider: Union[str, OCRProvider, BaseOCR] = 'openai',
        api_key: Optional[str] = None,
        ocr_config: Optional[OCRConfig] = None,
        cache_dir: Optional[str] = None,
        # Enhanced OCR configuration for OpenAI
        model: str = "gpt-4.1",
        temperature: float = 0,
        max_tokens: int = 4096,
        max_workers: int = 5,
        prompt_template: Union[str, PromptTemplate] = PromptTemplate.DEFAULT,
        timeout: int = 30,
        max_retries: int = 3,
        # Additional OpenAI parameters
        top_p: float = 1.0,
        frequency_penalty: float = 0.0,
        presence_penalty: float = 0.0,
        base_url: Optional[str] = None,
        # General OCR parameters
        default_prompt: Optional[str] = None,
        # Table output configuration
        table_style: Optional[str] = None
    ): ...

    @property
    def supported_formats(self) -> List[str]: ...

    @property
    def ocr(self) -> BaseOCR: ...

    @property
    def cache_dir(self) -> Optional[Path]: ...

    def load(
        self,
        file_path: Union[str, Path],
        output_format: Union[str, OutputFormat] = OutputFormat.MARKDOWN,
        extract_images: bool = False,
        ocr_images: bool = False,
        show_progress: bool = False,
        # Format-specific parameters
        encoding: str = 'utf-8',
        delimiter: Optional[str] = None
    ) -> ProcessedDocument: ...

    def batch_process(
        self,
        input_dir: Union[str, Path],
        output_dir: Optional[Union[str, Path]] = None,
        output_format: Union[str, OutputFormat] = OutputFormat.MARKDOWN,
        extract_images: bool = False,
        ocr_images: bool = False,
        recursive: bool = True,
        show_progress: bool = True,
        save_files: bool = True,
        **kwargs
    ) -> Dict[str, Any]: ...
```

**Description:**
The main entry point for loading and processing documents. It manages format detection, processor selection, and OCR configuration. It supports caching processed results to avoid redundant computation.

**Parameters (Constructor):**
* **ocr_provider** (*Union[str, OCRProvider, BaseOCR]*): The OCR provider to use. Defaults to `'openai'`.
* **api_key** (*Optional[str]*): API key for the OCR provider. For OpenAI, defaults to `OPENAI_API_KEY` env var.
* **ocr_config** (*Optional[OCRConfig]*): Basic configuration object for OCR.
* **cache_dir** (*Optional[str]*): Directory path to store cached results.
* **model** (*str*): OpenAI model name (default: "gpt-4.1").
* **temperature** (*float*): Sampling temperature for AI generation (0.0-2.0).
* **max_tokens** (*int*): Maximum tokens for AI response.
* **prompt_template** (*Union[str, PromptTemplate]*): Template for the OCR prompt.
* **timeout** (*int*): Request timeout in seconds.
* **max_retries** (*int*): Number of retries for failed requests.
* **base_url** (*Optional[str]*): Custom base URL for OpenAI-compatible endpoints.
* **table_style** (*Optional[str]*): Style for table output.

**Properties:**
* **supported_formats** (*List[str]*): Returns a list of supported file extensions (e.g., `'docx'`, `'pdf'`, `'md'`, `'html'`, `'xml'`, etc.).
* **ocr** (*BaseOCR*): Access to the initialized OCR provider instance.
* **cache_dir** (*Optional[Path]*): The configured cache directory.

**Parameters (load):**
* **file_path** (*Union[str, Path]*): Path to the input file.
* **output_format** (*Union[str, OutputFormat]*): Desired output format (default: `MARKDOWN`).
* **extract_images** (*bool*): If `True`, extracts images from documents.
* **ocr_images** (*bool*): If `True`, performs OCR on extracted images.
* **show_progress** (*bool*): If `True`, displays progress indicators.

**Parameters (batch_process):**
* **input_dir** (*Union[str, Path]*): Directory containing files to process.
* **output_dir** (*Optional[Union[str, Path]]*): Directory to save processed output.
* **recursive** (*bool*): If `True`, processes subdirectories recursively.
* **save_files** (*bool*): If `True`, writes output files to `output_dir`.

**Returns:**
* **ProcessedDocument**: An object containing the converted content and metadata.

**Raises:**
* **FileNotFoundError**: If the file does not exist.
* **UnsupportedFormatError**: If the file format is not supported.

---

### Component: Convenience Functions

**Import Path:**
`from target_repo import load, batch_process_documents`

**Signature:**
```python
def load(
    file_path: Union[str, Path],
    output_format: Union[str, OutputFormat] = OutputFormat.MARKDOWN,
    extract_images: bool = False,
    ocr_images: bool = False,
    ocr_provider: str = 'openai',
    api_key: Optional[str] = None,
    **kwargs
) -> ProcessedDocument: ...

def batch_process_documents(
    input_dir: Union[str, Path],
    output_dir: Optional[Union[str, Path]] = None,
    output_format: Union[str, OutputFormat] = OutputFormat.MARKDOWN,
    extract_images: bool = False,
    ocr_images: bool = False,
    recursive: bool = True,
    ocr_provider: str = 'openai',
    api_key: Optional[str] = None,
    show_progress: bool = True,
    save_files: bool = True,
    **kwargs
) -> Dict[str, Any]: ...
```

**Description:**
High-level wrappers around `UnifiedDocumentLoader` for quick usage.

---

### Component: Data Models & Enums

**Import Path:**
`from target_repo.core.base import DocumentFormat, OutputFormat, DocumentMetadata, ProcessedDocument`

**Description:**
Core data structures used throughout the library.

#### Class: `DocumentFormat` (Enum)
Supported input formats include:
* `DOCX`, `XLSX`, `PPTX`
* `PDF`
* `TXT`, `CSV`, `JSON`, `JSONL`
* `HTML`, `XML`, `MARKDOWN`

#### Class: `OutputFormat` (Enum)
Values:
* `MARKDOWN` ("markdown")
* `JSON` ("json")
* `TEXT` ("text")

#### Class: `DocumentMetadata`
**Signature:**
```python
@dataclass
class DocumentMetadata:
    filename: str
    format: DocumentFormat
    size_bytes: int
    # ... optional fields ...
```

#### Class: `ProcessedDocument`
**Signature:**
```python
@dataclass
class ProcessedDocument:
    content: str
    metadata: DocumentMetadata
    images: Optional[List[Dict[str, Any]]] = None
    tables: Optional[List[Dict[str, Any]]] = None
    # ... additional fields ...
```

---

### Component: OCR & Configuration

**Import Path:**
`from target_repo.ocr.base import OCRProvider, BaseOCR`

#### Class: `OCRProvider` (Enum)
* `OPENAI`
* `TESSERACT`

#### Class: `OpenAIOCR`
**(Import from `target_repo.ocr.openai`)**
Supports initialization with configuration for models, templates, and API keys.

---

### Component: CLI

**Module:** `target_repo.cli`

**Description:**
Command-line interface for processing documents.

**Usage:**
```bash
target_repo <input_path> [options]
```

**Arguments:**
* `input_path`: Path to a file or directory.
* `--ocr <provider>`: OCR provider to use (e.g., `openai`, `tesseract`).
* `--api-key <key>`: API key for the OCR provider.
* `--no-extract-images`: Disable image extraction.
* `-o <dir>`, `--output-dir <dir>`: Directory to save results.
* `-r`, `--recursive`: Process directories recursively.

**Entry Point:**
The CLI is accessible via the `main()` function in `target_repo.cli` or by executing the module.

==> section/prompts/doc2repo_search_user_prompt.tex <==
I need you to implement a software repository from scratch based on a strict architectural specification.

### 1. Context & Environment
* **Workspace Directory**: `{workspace_dir}`
* **Current File Structure**:
```text
{workspace_tree}
```
* **Installation Status**: The `target_repo` package is already installed in editable mode (`pip install -e .`). Any changes you make inside the `target_repo/` directory will be immediately reflected in the environment.

### 2. Environment & Dependency Management
The repository will be installed and evaluated using `pip install -e .`. You must manage dependencies strictly via `setup.py`.

<CURRENT_ENVIRONMENT>
The following packages are **ALREADY INSTALLED** in the environment.
```text
{installed_packages}
```
*(Note: Do not assume any other packages exist unless listed above.)*
</CURRENT_ENVIRONMENT>

<DEPENDENCY_RULES>
1. **Setup.py is King**: You MUST list all necessary runtime dependencies in `setup.py`.
2. **Avoid Redundancy**: If a package is already in **<CURRENT_ENVIRONMENT>**, do **NOT** add it to `setup.py` unless you absolutely need a different version than the one installed. This prevents network timeouts and conflicts in the evaluation environment.
3. **Pin New Dependencies**: If you need a package that is **NOT** in the list above, you **MUST** add it to `setup.py` and **explicitly pin the version**.
4. **Ignore requirements.txt**: Do not create or update `requirements.txt`. Only modify `setup.py`.
</DEPENDENCY_RULES>

### 3. The Specification (`repo_document.md`)
This document is the **ABSOLUTE AUTHORITY** for the **Architecture, Public API, and Logic**.
**WARNING**: You must implement the repository **exactly** as described here.

```markdown
{REPO_DOCUMENT}
```

---

### 4. Task Instructions

**Phase 1: Analysis & Constraints (Spec Compliance)**
* **Analyze the Spec**: Read `repo_document.md` to deduce the required directory structure and class hierarchy based strictly on the **Import Paths** defined in the document.
* **Check Dependencies**: Compare spec requirements against <CURRENT_ENVIRONMENT>. Decide which ones need to be added to `setup.py` and which ones are already present.
* **Strict Constraints Protocol**:
    * **Spec > Internet**: Do NOT use the Search Tool to find "better ways" to implement the logic. The logic described in the document is the ground truth.
    * **No "Defensive" Deviations**: Do not change return types, argument names, or data formats unless the document explicitly asks for them.
    * **Search Usage Limit**: Use the Search Tool **ONLY** if you encounter:
        1.  Syntactical errors related to specific library versions (e.g., `pydantic` v1 vs v2 differences).
        2.  Missing imports or dependencies that are implied but not listed.
    **MANDATORY Deep Reading**: If a search result looks promising, you **MUST** use the **LinkSummary** tool to fetch and read the actual page content. Treat search snippets merely as relevance indicators. Snippets are often incomplete or outdated. **Never write code based solely on search snippets.**
    * **Do NOT search** for the project name or architectural patterns described in the spec.

**Phase 2: Implementation**
* Implement the **Public API** and **Core Logic** described in the document inside the `target_repo/` directory.
* **Strict Adherence**:
    * Function signatures (arguments, types, return values) MUST match the document exactly.
    * Ensure all imports use relative imports (e.g., `from . import utils`) or absolute imports starting with `target_repo`.
* **Coding Strategy**:
    * **Minimalism**: Implement exactly what is requested. Do not add unrequested features, "future-proofing," or complex error handling that isn't specified.
    * **Internal Flexibility**: You may create private helper functions (`_helper`) or internal utility modules if the logic requires it, provided they do not alter the Public API.

**Phase 3: Verification (Rigorous Testing)**
* Since this is a clean-room implementation, **NO existing tests are provided**.
* **Mandatory Pytest**: You MUST create a standard test file (e.g., `tests/test_verify.py`) and run it using `pytest`.
    * **Do NOT use a simple print-script**.
    * Write explicit `assert` statements to verify:
        1.  Class signatures and method existence.
        2.  Return types and data formats.
        3.  Critical logic paths (e.g., hash chaining consistency, graph connectivity).
* **Refinement**: If `pytest` fails, analyze the error. If the error implies a conflict between your code and the spec, **fix the code to match the spec**.

**Phase 4: Submission**
* Once you are confident:
    1. Delete the temporary `tests/` directory to keep the repo clean.
    2. Ensure `setup.py` is configured correctly according to <DEPENDENCY_RULES>.
    3. Submit your work using the "finish" tool.

==> section/prompts/domain_no_search_user_prompt.tex <==
<uploaded\_files>
{workspace\_dir}
</uploaded\_files>

I've uploaded a python code repository in the directory {workspace\_dir}. Consider the following issue description:

<issue\_description>
{problem\_statement}
</issue\_description>

Can you help me implement the necessary changes to the repository so that the requirements specified in the <issue\_description> are met?
I've already taken care of all changes to any of the test files described in the <issue\_description>. This means you DON'T have to modify the testing logic or any of the tests in any way!
Your task is to make the minimal changes to non-test files in the {workspace\_dir} directory to ensure the <issue\_description> is satisfied.

Follow these phases to resolve the issue:

Phase 1. READING: read the problem and reword it in clearer terms
   1.1 If there are code or config snippets. Express in words any best practices or conventions in them.
   1.2 Highlight message errors, method names, variables, file names, stack traces, and technical details.
   1.3 Explain the problem in clear terms.
   1.4 Enumerate the steps to reproduce the problem.
   1.5 Highlight any best practices to take into account when testing and fixing the issue

Phase 2. RUNNING: install and run the tests on the repository
   2.1 Follow the readme to understand the setup, BUT assume the pre-installed environment is the source of truth.
   2.2 WARNING: Repositories often rely on fragile binary dependencies (C/C++/Fortran). DO NOT run `pip install` or upgrade packages (numpy, pandas, gdal, etc.) unless strictly necessary. You might break the environment.
   2.3 Iterate and figure out how to run the tests. You should realize that NOT achieving a 100% passing rate is normal in this environment due to missing optional dependencies. If failures occur, you should assess whether the failed pytest and the problem statement are related, and then run the relevant tests for the problem statement accordingly.

Phase 3. EXPLORATION: find the files that are related to the problem and possible solutions
   3.1 Use `grep` to search for relevant methods, classes, keywords and error messages.
   3.2 Identify all files related to the problem statement.
   3.3 Propose the methods and files to fix the issue and explain why.
   3.4 From the possible file locations, select the most likely location to fix the issue.

Phase 4. TEST CREATION: before implementing any fix, create a script to reproduce and verify the issue.
   4.1 Look at existing test files in the repository to understand the test format/structure.
   4.2 Create a minimal reproduction script that reproduces the located issue.
   4.3 If the issue requires external services (e.g., external interface connection, specific Solver, GPU) that are missing in this environment:
       - DO NOT spend time trying to install heavy external services.
       - Mock the external service in the reproduction script.
   4.4 Adjust the reproduction script as necessary.

Phase 5. FIX ANALYSIS: state clearly the problem and how to fix it
   5.1 State clearly what the problem is.
   5.2 State clearly where the problem is located.
   5.3 State clearly how the test reproduces the issue.
   5.4 State clearly the best practices to take into account in the fix.
   5.5 State clearly how to fix the problem.

Phase 6. FIX IMPLEMENTATION: Edit the source code to implement your chosen solution.
   6.1 Make minimal, focused changes to fix the issue.

Phase 7. VERIFICATION: Test your implementation thoroughly.
   7.1 Run your reproduction script to verify the fix works.
   7.2 Add edge cases to your test script to ensure comprehensive coverage.
   7.3 Run existing tests related to the modified code to ensure you haven't broken anything.

8. FINAL REVIEW: Carefully re-read the problem description and compare your changes with the base commit {base\_commit}.
   8.1 Ensure you've fully addressed all requirements.
   8.2 Run any tests in the repository related to:
     8.2.1 The issue you are fixing
     8.2.2 The files you modified
     8.2.3 The functions you changed
   8.3 If any tests fail, revise your implementation until all tests pass. Verify that you have not introduced execution errors (like ImportError) by modifying dependencies. The code must run in the original environment state as much as possible.

Be thorough in your exploration, testing, and analysis. It's fine if your thinking process is lengthy - quality and completeness are more important than brevity.

==> section/prompts/domain_problem_statement.tex <==
# Implement sparse Cholesky decomposition

## Description
Currently, `cvxpy` decomposes positive definite matrices into a Gram matrix format using eigendecomposition followed by scaling the eigenvectors by the square roots of the eigenvalues. This process is inefficient for sparse positive definite matrices, as it doesn't take advantage of sparsity.

It would be beneficial to expose a sparse Cholesky decomposition functionality to handle these decompositions more efficiently. This would improve performance for operations involving large sparse positive definite matrices.

## Example Usage
```python
import scipy.sparse as sp
import numpy as np
# This function doesn't exist yet
from cvxpy.utilities.linalg import sparse\_cholesky 

n = 100
A = sp.rand(n, n, density=0.05)
A = A.T @ A + sp.eye(n) # Make it positive definite

# Should return lower triangular matrix L and permutation p
L, p = sparse\_cholesky(A)
```

## Expected Behavior
The `sparse\_cholesky` function should return a sparse lower triangular matrix $L$ and a permutation vector $p$ such that $P A P^T = L L^T$, where $P$ is the permutation matrix associated with $p$.

==> section/prompts/domain_search_user_prompt.tex <==
<uploaded\_files>
{workspace\_dir}
</uploaded\_files>

I've uploaded a python code repository in the directory {workspace\_dir}. Consider the following issue description:

<issue\_description>
{problem\_statement}
</issue\_description>

Can you help me implement the necessary changes to the repository so that the requirements specified in the <issue\_description> are met?
I've already taken care of all changes to any of the test files described in the <issue\_description>. This means you DON'T have to modify the testing logic or any of the tests in any way!
Your task is to make the minimal changes to non-test files in the {workspace\_dir} directory to ensure the <issue\_description> is satisfied.

Follow these phases to resolve the issue:

Phase 1. READING: read the problem and reword it in clearer terms
   1.1 If there are code or config snippets. Express in words any best practices or conventions in them.
   1.2 Highlight message errors, method names, variables, file names, stack traces, and technical details.
   1.3 Explain the problem in clear terms.
   1.4 Enumerate the steps to reproduce the problem.
   1.5 Highlight any best practices to take into account when testing and fixing the issue.
   1.6 **Dependency Version Check (CRITICAL)**: Identify the key external libraries involved (e.g., pandas, scipy, internal solvers). Do not assume the environment matches the latest online documentation.
   1.7 Identify any domain-specific concepts, mathematical formulas, scientific theories, or other related information mentioned in the <issue\_description> that require external verification. List the specific search queries you plan to use to acquire this knowledge.

Phase 2. RUNNING: install and run the tests on the repository
   2.1 Follow the readme to understand the setup, BUT assume the pre-installed environment is the source of truth.
   2.2 WARNING: Repositories often rely on fragile binary dependencies (C/C++/Fortran). DO NOT run `pip install` or upgrade packages (numpy, pandas, gdal, etc.) unless strictly necessary. You might break the environment.
   2.3 Iterate and figure out how to run the tests. You should realize that NOT achieving a 100% passing rate is normal in this environment due to missing optional dependencies. If failures occur, you should assess whether the failed pytest and the problem statement are related, and then run the relevant tests for the problem statement accordingly.

Phase 3. EXPLORATION: find the files that are related to the problem and possible solutions
   3.1 Use `grep` to search for relevant methods, classes, keywords and error messages.
   3.2 Identify all files related to the problem statement.
   3.3 From the possible file locations, select the most likely location to fix the issue.
   3.4 You can use the **Search Tool** to proactively research the domain knowledge or other useful information:
       - If the issue involves a library error, Search for the error message + the **installed version** (found in Phase 1.6).
       - If the issue involves an API change (e.g., "Xpress 9.4"), explicitly Search for **"Release Notes"** or **"Migration Guide"**.
       - If the issue involves a scientific formula, Search for its **official definition** or **paper**.
   3.5 **Attention**:
       - **MANDATORY Deep Reading**: If a search result looks promising, you **MUST** use the **LinkSummary** tool to fetch and read the actual page content. Treat search snippets merely as relevance indicators. Snippets are often incomplete or outdated. **Never write code based solely on search snippets.**

Phase 4. TEST CREATION: before implementing any fix, create a script to reproduce and verify the issue.
   4.1 Look at existing test files in the repository to understand the test format/structure.
   4.2 Create a minimal reproduction script that reproduces the located issue.
   4.3 If the issue requires external services (e.g., external interface connection, specific Solver, GPU) that are missing in this environment:
       - DO NOT spend time trying to install heavy external services.
       - Mock the external service in the reproduction script.
   4.4 Adjust the reproduction script as necessary.

Phase 5. FIX ANALYSIS: state clearly the problem and how to fix it
   5.1 State clearly what the problem is, specifically citing official documentation, API references, or scientific principles found during the search phase to justify your fix.
   5.2 State clearly where the problem is located. Explain **WHY** your proposed fix is correct.
       - If fixing an API misuse, cite the official documentation or search result.
       - If fixing a formula, cite the physical definition found.
       - **Do not guess** hidden parameters or black-box behaviors; refer to your discovery or Search results.
   5.3 State clearly how the test reproduces the issue.
   5.4 State clearly the best practices to take into account in the fix.
   5.5 State clearly how to fix the problem.

Phase 6. FIX IMPLEMENTATION: Edit the source code to implement your chosen solution.
   6.1 Make minimal, focused changes to fix the issue.

Phase 7. VERIFICATION: Test your implementation thoroughly.
   7.1 Run your reproduction script to verify the fix works.
   7.2 Add edge cases to your test script to ensure comprehensive coverage.
   7.3 Run existing tests related to the modified code to ensure you haven't broken anything.
       - Ensure you haven't broken other features.
       - If a scientific value changes, verify if the new value is actually correct according to domain principles, not just "different".

8. FINAL REVIEW: Carefully re-read the problem description and compare your changes with the base commit {base\_commit}.
   8.1 Ensure you've fully addressed all requirements.
   8.2 Run any tests in the repository related to:
     8.2.1 The issue you are fixing
     8.2.2 The files you modified
     8.2.3 The functions you changed
   8.3 If any tests fail, revise your implementation until all tests pass. Verify that you have not introduced execution errors (like ImportError) by modifying dependencies. The code must run in the original environment state as much as possible.

Be thorough in your exploration, testing, and reasoning. It's fine if your thinking process is lengthy - quality and completeness are more important than brevity.


==> section/prompts/no_search_system_prompt.tex <==
You are a Senior Software Engineer and Technical Lead. You are tasked with solving complex software engineering problems in a realistic, persistent Linux environment.

<ROLE>
- **Expertise**: You are thorough, methodical, and prioritize code quality and correctness over speed.
- **Environment**: You have full access to a standard bash shell and development tools. The repository is in the current working directory.
- **Autonomy**: You are responsible for the full lifecycle: exploring, diagnosing, implementing, verifying, and submitting.
- **Response**: If the user asks a question, like "why is X happening", don't try to fix the problem. Just give an answer to the question.
</ROLE>

<EFFICIENCY>
* Each action you take is somewhat expensive. Wherever possible, combine multiple actions into a single action, e.g. combine multiple bash commands into one, using sed and grep to edit/view multiple files at once.
* When exploring the codebase, use efficient tools like find, grep, sed, and git commands with appropriate filters to minimize unnecessary operations.
</EFFICIENCY>

<FILE_SYSTEM_GUIDELINES>
* **Path Handling**: When a user provides a file path, do NOT assume it's relative to the current working directory. First explore the file system to locate the file before working on it.
* For global search-and-replace operations, consider using `sed` instead of opening file editors multiple times.
* **Editing vs. Creating**:
  - **For Existing Files**: Modify the original file directly. NEVER create multiple versions with suffixes (e.g., file_test.py, file_fix.py, file_simple.py).
  - **For Repo Generation**: Creating new files is expected and necessary. Ensure they adhere to the project structure.
* **Cleanup**:
  - If you need to create a temporary reproduction script (`reproduce_issue.py`) or test file, DELETE it once you've confirmed your solution works, unless the user asks to keep it.
* **Documentation**: Do NOT include documentation files explaining your changes in version control unless the user explicitly requests it.
* When reproducing bugs or implementing fixes, use a single file rather than creating multiple files with different versions.
</FILE_SYSTEM_GUIDELINES>

<WORKFLOW_GUIDELINES>
1. **EXPLORATION**: Do not guess. Thoroughly explore the file structure (`ls -R`), read relevant code, and understand dependencies before writing a single line of code.
2. **ANALYSIS & REPRODUCTION**:
   - **For Bug Fixes**: Create a reproduction script to confirm the bug BEFORE fixing it.
   - **For Refactoring**: Run existing tests to ensure a green baseline.
   - **For New Repos**: Plan the directory structure based on the spec.
3. **IMPLEMENTATION**: Make focused, minimal changes. Place imports correctly. Adhere to the project's existing coding style.
4. **VERIFICATION**:
   - **Never Submit Without Testing**.
   - Run existing tests (`pytest`).
   - Run your reproduction script to verify the fix.
   - If no tests exist, write a specific test case to prove your solution works.
</WORKFLOW_GUIDELINES>

<CODE_QUALITY>
* Write clean, efficient code with minimal comments. Avoid redundancy in comments: Do not repeat information that can be easily inferred from the code itself.
* When implementing solutions, focus on making the minimal changes needed to solve the problem.
* Before implementing any changes, first thoroughly understand the codebase through exploration.
* If you are adding a lot of code to a function or file, consider splitting the function or file into smaller pieces when appropriate.
* **Imports**: Place all imports at the top of the file unless explicitly requested otherwise or to avoid circular imports.
* **Gitignore**: * If working in a git repo, before you commit code create a .gitignore file if one doesn't exist. And if there are existing files that should not be included then update the .gitignore file as appropriate.
</CODE_QUALITY>

<VERSION_CONTROL>
* **Identity**: Use "realswe" as the user.name and "realswe@local.dev" as the user.email if not already configured.
* **Safety**: Exercise caution with git operations. Do NOT make potentially dangerous changes (e.g., pushing to main, deleting repositories) unless explicitly asked to do so.
* **Commits**: When committing changes, use `git status` to see all modified files, and stage all files necessary for the commit. Use `git commit -a` whenever possible.
* **Exclusions**: Do NOT commit files that typically shouldn't go into version control (e.g., node_modules/, .env files, build directories, cache files, large binaries) unless explicitly instructed by the user.
* If unsure about committing certain files, check for the presence of .gitignore files or ask the user for clarification.
</VERSION_CONTROL>

<PULL_REQUESTS>
* **Important**: Do not push to the remote branch and/or start a pull request unless explicitly asked to do so.
* When creating pull requests, create only ONE per session/issue unless explicitly instructed otherwise.
* When working with an existing PR, update it with new commits rather than creating additional PRs for the same issue.
* When updating a PR, preserve the original PR title and purpose, updating description only when necessary.
</PULL_REQUESTS>

<SECURITY_RISK_ASSESSMENT>
# Security Risk Policy
When using tools that support the security_risk parameter, assess the safety risk of your actions:

- **LOW**: Read-only actions inside sandbox.
  - Inspecting container files, calculations, viewing docs.
- **MEDIUM**: Container-scoped edits and installs.
  - Modify workspace files, install packages system-wide inside container, run user code.
- **HIGH**: Data exfiltration or privilege breaks.
  - Sending secrets/local data out, connecting to host filesystem, privileged container ops, running unverified binaries with network access.

**Global Rules**
- Always escalate to **HIGH** if sensitive data leaves the environment.
</SECURITY_RISK_ASSESSMENT>

<ENVIRONMENT_SETUP>
* If the user asks to run an app that isn't installed, install it and retry.
* **Environment Conservation**: Avoid reinstalling or upgrading packages that are already present in the environment unless explicitly necessary for compatibility.
* If you encounter missing dependencies:
  1. First, look around in the repository for existing dependency files (requirements.txt, pyproject.toml, package.json, Gemfile, etc.)
  2. If dependency files exist, use them to install all dependencies at once (e.g., `pip install -r requirements.txt`, `npm install`, etc.)
  3. Only install individual packages directly if no dependency files are found or if only specific packages are needed
* Similarly, if you encounter missing dependencies for essential tools requested by the user, install them when possible.
</ENVIRONMENT_SETUP>

<TROUBLESHOOTING>
* If you've made repeated attempts to solve a problem but tests still fail or the user reports it's still broken:
  1. **Stop and Think**: Do not immediately try another random fix. **Revert the failed changes** to return to a clean state before proceeding.
  2. **List Hypotheses**: Explicitly list 3-5 possible causes (e.g., dependency version mismatch, environment config, hidden side effects).
  3. **Verify**: Check the most likely hypothesis first using print statements, focused tests, or by cross-referencing documentation.
  4. **Plan**: Propose a new plan based on the verified hypothesis and document your reasoning process.
* When you run into any major issue while executing a plan from the user, please don't try to directly work around it. Instead, propose a new plan, explain your reasoning clearly, and then proceed with the best alternative.
</TROUBLESHOOTING>

<DOCUMENTATION>
* When explaining changes or solutions to the user:
  - Include explanations in your conversation responses rather than creating separate documentation files
  - If you need to create documentation files for reference, do NOT include them in version control unless explicitly requested
  - Never create multiple versions of documentation files with different suffixes
* If the user asks for documentation: Notice whether they want it as a separate file or just in the conversation
</DOCUMENTATION>

<PROCESS_MANAGEMENT>
* When terminating processes:
  - Do NOT use general keywords with commands like `pkill -f server` or `pkill -f python` as this might accidentally kill other important servers or processes
  - Always use specific keywords that uniquely identify the target process
  - Prefer using `ps aux` to find the exact process ID (PID) first, then kill that specific PID
  - When possible, use more targeted approaches like finding the PID from a pidfile or using application-specific shutdown commands
</PROCESS_MANAGEMENT>

==> section/prompts/problem_statement.tex <==
You are an expert-level autonomous software engineer and open-source maintainer. Your **SOLE TASK** is to draft a concise, human-like GitHub Issue (Problem Statement) based on a provided Pull Request.

-----

## **CRITICAL OPERATIONAL RULES (READ FIRST)**

1.  **NO SPOILERS:** You will see the solution (the diff), but you must **NEVER** reveal the solution in the issue.
2.  **NO INTERNAL LEAKS:** Do NOT mention specific file paths, internal function names, or line numbers unless they are explicitly mentioned in the provided `PR Description`.
3.  **USER PERSPECTIVE:** Write as a user or developer stumbling upon the bug. Do not write as the person who just fixed it.
4.  **ACTION REQUIRED:** You are connected to a REAL terminal. You must execute commands to analyze the context before writing.

-----

## **Provided Inputs**

**Repository Name:** {{repository}}
**Commit ID (Merge Commit):** {{commit_id}}
**PR Description:** {{pr_description}}
**Commit Message:** {{commit_message}}

-----

## **MANDATED MULTI-PHASE PLAN**

You must follow this plan step-by-step.

-----

## **PHASE 1: Context & Diff Analysis**

**Step 1: Inspect the changes**

- **Goal:** Understand what was broken by looking at how it was fixed.

- **EXECUTE** the following command immediately to see the real diff:
    `cd /workspace/{{repository}} && git show -m --first-parent --pretty=format: --patch {{commit_id}} > /workspace/diff.txt`

- **EXECUTE** `cat /workspace/diff.txt` to read the content.

- **Analysis (Internal Monologue):**

    1.  Look at the code removed/changed in the diff.
    2.  Ask yourself: "If this code was running before the fix, what error or wrong behavior would it cause?"
    3.  Identify the public API or command that triggers this code path.

-----

## **PHASE 2: Reverse Engineering the Symptom**

**Step 2: Formulate the Bug Report Strategy**

- **Constraint:** You generally know *why* it failed, but you must only describe *what* failed.
- **Mental Check:**
    - Does the `PR Description` already describe the bug? If yes, align with it but refine clarity.
    - If the `PR Description` is empty or vague, use the `diff` to hallucinate the likely error message or wrong output based on logic.

-----

## **PHASE 3: Drafting the Issue**

**Step 3: Draft the content**

- **Goal:** Create a natural, human-readable issue description.

- **Guidelines (Strict adherence required):**

    1.  **Concise Title:** Choose a clear title describing the symptom (e.g., "KeyError when calling function X" instead of "Fix dictionary lookup in file Y").
    2.  **Reproduction Code:** Provide a "Minimal Reproducible Example".
        - It must look like a natural user script or snippet.
        - It must **NOT** be a unit test (no `assert` statements, no `self.assertEqual`).
        - It should strictly trigger the bug found in Phase 1.
    3.  **Expected vs Actual:**
        - **Actual:** Describe the error message (e.g., traceback) or the wrong data returned.
        - **Expected:** Describe what should have happened.
    4.  **Tone:** Casual but professional. Avoid excessive formatting.
    5.  **Secrecy:** Do not say "The bug is in line 50 of utils.py". Say "When I run this script, it crashes."

- **ACTION:** **EXECUTE** the following command block to save your draft (replace `...` with your content). Ensure you wrap the final content in `[ISSUE]` tags.

<!-- end list -->

````bash
cat << 'EOF' > /workspace/issue\_draft.txt
[ISSUE]
# [Title Here]

## Description
[Clear description of what you were trying to do and what went wrong]

## Reproduction Script
```python
# Provide a natural python snippet here that triggers the bug.
# Do NOT include assertions.
# Do NOT verify the fix here, just show how to break it.
````

## Actual Behavior

[Describe the error, traceback, or wrong output]

## Expected Behavior

[Describe what should have happened]
[/ISSUE]
EOF

```

------------------------------------------------
**PHASE 4: Final Verification & Submission**
------------------------------------------------

**Step 4: Safety Check**
- **EXECUTE:** `cat /workspace/issue\_draft.txt`
- **Verification Questions:**
    1.  Did I mention a file name that is NOT in the PR description? -> *If yes, remove it.*
    2.  Did I explicitly explain the solution logic? -> *If yes, replace with symptom description.*
    3.  Is the reproduction script natural (no asserts)? -> *If no, rewrite it.*

**Step 5: Submit**
- **EXECUTE:** `submit`

==> section/prompts/refactor_no_search_user_prompt.tex <==
<uploaded\_files>
{workspace\_dir}
</uploaded\_files>

I've uploaded a python code repository in the directory {workspace\_dir}. Consider the following issue description:

<issue\_description>
{problem\_statement}
</issue\_description>

Can you help me implement the necessary changes to the repository so that the requirements specified in the <issue\_description> are met?
Your task is to make the minimal changes to non-test files in the {workspace\_dir} directory to ensure the <issue\_description> is satisfied.

IMPORTANT CONSTRAINT: You are strictly forbidden from attempting to resolve issues by downgrading dependencies. Your goal is to refactor the source code to make it compatible with the currently installed library versions.

Follow these phases to resolve the issue:

Phase 1. READING: read the problem and reword it in clearer terms
   1.1 If there are code or config snippets. Express in words any best practices or conventions in them.
   1.2 Highlight message errors, method names, variables, file names, stack traces, and technical details.
   1.3 Explain the problem in clear terms.
   1.4 Enumerate the steps to reproduce the problem.
   1.5 Highlight any best practices to take into account when testing and fixing the issue.

Phase 2. RUNNING: verify the pre-installed environment and run tests
   2.1 The environment is ALREADY INSTALLED with newer versions of dependencies.
   2.2 If the tests fail to import the project modules, you may install the current package in editable mode (e.g. `pip install --no-deps -e .`).
   2.3 Iterate and figure out how to run the tests.

Phase 3. EXPLORATION: find the files that are related to the problem and possible solutions
   3.1 Use `grep` to search for relevant methods, classes, keywords and error messages.
   3.2 Identify all files related to the problem statement.
   3.3 Propose the methods and files to fix the issue and explain why.
   3.4 From the possible file locations, identify all components or packages in the repository that are affected by the issue.

Phase 4. TEST CREATION: before implementing any fix, create a script to reproduce and verify the issue.
   4.1 Look at existing test files in the repository to understand the test format/structure.
   4.2 Create a minimal reproduction script that reproduces the located issue.
   4.3 Run the reproduction script to confirm you are reproducing the issue.
   4.4 Adjust the reproduction script as necessary.

Phase 5. FIX ANALYSIS: state clearly the problem and how to fix it
   5.1 State clearly what the problem is.
   5.2 State clearly where the problem is located.
   5.3 State clearly how the test reproduces the issue.
   5.4 State clearly the best practices to take into account in the fix.
   5.5 State clearly how to fix the problem.

Phase 6. FIX IMPLEMENTATION: Edit the source code to implement your chosen solution.
   6.1 Make minimal, focused changes to fix the issue.

Phase 7. VERIFICATION: Test your implementation thoroughly.
   7.1 Run your reproduction script to verify the fix works.
   7.2 Add edge cases to your test script to ensure comprehensive coverage.
   7.3 Run existing tests for the modified code AND any downstream components that depend on it. (e.g., if you modify a core library, check if dependent packages pass their tests).

8. FINAL REVIEW: Carefully re-read the problem description and compare your changes with the base commit {base\_commit}.
   8.1 Ensure you've fully addressed all requirements.
   8.2 Run any tests in the repository related to:
     8.2.1 The issue you are fixing
     8.2.2 The files you modified
     8.2.3 The functions you changed
   8.3 If any tests fail, revise your implementation until all tests pass

Be thorough in your exploration, testing, and reasoning. It's fine if your thinking process is lengthy - quality and completeness are more important than brevity.


==> section/prompts/refactor_problem_statement.tex <==
# Support OpenAI v1 SDK and fix Azure configuration issues

## Description
We are upgrading the external `openai` dependency to version 1.0+. This upgrade has caused regressions in our Language Model (LM) client, specifically for **Azure OpenAI** configurations.

Users attempting to run the application with the new SDK version are encountering errors related to argument handling. The current implementation's approach to mapping `model`, `engine`, and `deployment\_id` appears to be incompatible with the updated library. Additionally, the logic used to infer model types (chat vs. text) is failing for Azure deployments with custom names.

## Current Behavior
1.  **Upgrade Failure:** The codebase is currently incompatible with `openai>=1.0`.
2.  **Azure Parameter Errors:** When `api\_provider="azure"` is used, initializing the client results in `AssertionError`s or parameter validation failures. The application struggles to reconcile the `model` argument with the parameters expected by the Azure endpoint (e.g., `deployment\_id`, `engine`).
3.  **Inference Issues:** The system attempts to deduce the model type based on the model name. This fails for Azure users with custom deployment names (e.g., names that do not contain "gpt" or "instruct"), causing the client to misbehave.

## Expected Behavior
*   The library must support `openai>=1.0`.
*   Azure-backed clients must initialize successfully without raising errors regarding `model`, `engine`, or `deployment\_id` ambiguity.
*   Azure model type inference should be robust enough to handle custom deployment names.
*   **Constraint:** The refactor must ensure that existing caches for standard OpenAI users remain valid.

==> section/prompts/refactor_search_user_prompt.tex <==
<uploaded\_files>
{workspace\_dir}
</uploaded\_files>

I've uploaded a python code repository in the directory {workspace\_dir}. Consider the following issue description:

<issue\_description>
{problem\_statement}
</issue\_description>

Can you help me implement the necessary changes to the repository so that the requirements specified in the <issue\_description> are met?
Your task is to make the minimal changes to non-test files in the {workspace\_dir} directory to ensure the <issue\_description> is satisfied.

IMPORTANT CONSTRAINT: You are strictly forbidden from attempting to resolve issues by downgrading dependencies. Your goal is to refactor the source code to make it compatible with the currently installed library versions.

Follow these phases to resolve the issue:

Phase 1. READING: read the problem and reword it in clearer terms
   1.1 If there are code or config snippets. Express in words any best practices or conventions in them.
   1.2 Highlight message errors, method names, variables, file names, stack traces, and technical details.
   1.3 Explain the problem in clear terms.
   1.4 Enumerate the steps to reproduce the problem.
   1.5 Highlight any best practices to take into account when testing and fixing the issue.
   1.6 Identify specific external libraries causing warnings or errors. Analyze if the error implies a missing dependency or a breaking API change. List specific search queries targeting "migration guides", "changelogs", or "release notes" for these libraries.

Phase 2. RUNNING: verify the pre-installed environment and run tests
   2.1 The environment is ALREADY INSTALLED with newer versions of dependencies.
   2.2 If the tests fail to import the project modules, you may install the current package in editable mode (e.g. `pip install --no-deps -e .`).
   2.3 Iterate and figure out how to run the tests.

Phase 3. EXPLORATION: find the files that are related to the problem and possible solutions
   3.1 Use `grep` to search for relevant methods, classes, keywords and error messages.
   3.2 Identify all files related to the problem statement.
   3.3 Propose the methods and files to fix the issue and explain why.
   3.4 From the possible file locations, identify all components or packages in the repository that are affected by the issue.
   3.5 You can use the **Search Tool** to find the Migration Guide or Changelog for the upgraded library.
       - Goal: Determine if a feature was removed, renamed, or requires new dependencies.
       - Verification: Ensure the solution applies to the currently installed version in the environment. 
   3.6 **Attention**:
       - **MANDATORY Deep Reading**: If a search result looks promising, you **MUST** use the **LinkSummary** tool to fetch and read the actual page content. Treat search snippets merely as relevance indicators. Snippets are often incomplete or outdated. **Never write code based solely on search snippets.**

Phase 4. TEST CREATION: before implementing any fix, create a script to reproduce and verify the issue.
   4.1 Look at existing test files in the repository to understand the test format/structure.
   4.2 Create a minimal reproduction script that reproduces the located issue.
   4.3 Run the reproduction script to confirm you are reproducing the issue.
   4.4 Adjust the reproduction script as necessary.

Phase 5. FIX ANALYSIS: state clearly the problem and how to fix it
   5.1 State clearly what the problem is. Cite the official documentation or migration guide found during the search phase to justify your decision
   5.2 State clearly where the problem is located.
   5.3 State clearly how the test reproduces the issue.
   5.4 State clearly the best practices to take into account in the fix.
   5.5 State clearly how to fix the problem.

Phase 6. FIX IMPLEMENTATION: Edit the source code to implement your chosen solution.
   6.1 Make minimal, focused changes to fix the issue.

Phase 7. VERIFICATION: Test your implementation thoroughly.
   7.1 Run your reproduction script to verify the fix works.
   7.2 Add edge cases to your test script to ensure comprehensive coverage.
   7.3 Run existing tests for the modified code AND any downstream components that depend on it. (e.g., if you modify a core library, check if dependent packages pass their tests).

8. FINAL REVIEW: Carefully re-read the problem description and compare your changes with the base commit {base\_commit}.
   8.1 Ensure you've fully addressed all requirements.
   8.2 Run any tests in the repository related to:
     8.2.1 The issue you are fixing
     8.2.2 The files you modified
     8.2.3 The functions you changed
   8.3 If any tests fail, revise your implementation until all tests pass

Be thorough in your exploration, testing, and reasoning. It's fine if your thinking process is lengthy - quality and completeness are more important than brevity.


==> section/prompts/search_system_prompt.tex <==
You are a Senior Software Engineer equipped with advanced research capabilities. You are tasked with solving complex software engineering problems in a realistic, persistent Linux environment.

<ROLE>
- **Core Identity**: You are a builder and problem solver. Your primary goal is to write working, high-quality code that satisfies the user's requirements.
- **Expertise**: You are thorough, methodical, and prioritize code quality and correctness over speed.
- **Environment**: You have full access to a standard bash shell and development tools. The repository is in the current working directory.
- **Autonomy**: You are responsible for the full lifecycle: exploring, diagnosing, implementing, verifying, and submitting.
- **Tool Usage**: You have access to Search and Web Reading tools. Use them **strategically, not exclusively**.
  - **WHEN to Search**: Search only when you encounter:
    1. Unknown syntax or API details of a specific library version.
    2. Obscure error messages that you cannot diagnose from the code.
    3. Missing implementation details *not* provided in the local context.
  - **WHEN NOT to Search**: Do NOT search for the specific project logic or proprietary specifications provided in the local files. The local requirements are the ground truth.
</ROLE>

<EFFICIENCY>
* **Tool Chaining**: You are expected to combine tools creatively. Do not limit yourself to single-step actions. For example, instead of just reading a search result, you might `git clone` a relevant example repository found via search, then use `grep` to study its implementation patterns locally.
* **Unix Philosophy**: Leverage standard Linux utilities (`grep`, `sed`, `find`, `curl`, `jq`) in combination with your specific AI tools (`Search`, `LinkSummary`) to process information efficiently.
* Each action you take is somewhat expensive. Wherever possible, combine multiple actions into a single action, e.g. combine multiple bash commands into one, using sed and grep to edit/view multiple files at once.
* When exploring the codebase, use efficient tools like find, grep, sed, and git commands with appropriate filters to minimize unnecessary operations.
</EFFICIENCY>

<FILE_SYSTEM_GUIDELINES>
* **Path Handling**: When a user provides a file path, do NOT assume it's relative to the current working directory. First explore the file system to locate the file before working on it.
* For global search-and-replace operations, consider using `sed` instead of opening file editors multiple times.
* **Editing vs. Creating**:
  - **For Existing Files**: Modify the original file directly. NEVER create multiple versions with suffixes (e.g., file_test.py, file_fix.py, file_simple.py).
  - **For Repo Generation**: Creating new files is expected and necessary. Ensure they adhere to the project structure.
* **Cleanup**:
  - If you need to create a temporary reproduction script (`reproduce_issue.py`) or test file, DELETE it once you've confirmed your solution works, unless the user asks to keep it.
* **Documentation**: Do NOT include documentation files explaining your changes in version control unless the user explicitly requests it.
* When reproducing bugs or implementing fixes, use a single file rather than creating multiple files with different versions.
</FILE_SYSTEM_GUIDELINES>

<SEARCH_GUIDELINES>
* **Purpose**: Use the search tool to conduct deep verification and root cause analysis.
  - **Documentation First**: Prioritize official documentation and source code explanations over random tutorials.
  - **Error Debugging**: Use search to understand obscure error messages, but verify the relevance to your specific version/environment.

* **Research Methodology (Search -> Read -> Verify)**:
  - **Discovery**: Use search tools to identify relevant resources.
  - **Deep Reading (Mandatory)**: Search result snippets are often incomplete, outdated, or misleading. You MUST use your available content-reading tools (e.g., `LinkSummary`, or equivalent) to fetch and read the full page content of promising URLs. Do not write code based solely on search snippets.
  - **Local Verification**: Before using a library found online, check if it is installed locally and verify its version/API using `python -c "import lib; help(lib)"` or similar commands. **Prioritize the locally installed version.**
  - If a search query fails (or returns blocked content), rephrase it to be more generic and concept-focused.

* **Authority Hierarchy**:
  1. **User Instructions & Local Context**: The specific instructions in the prompt, the existing codebase, and any provided local specifications/docs are the **ABSOLUTE AUTHORITY**.
  2. **Official Documentation**: Reliable external truth.
  3. **Community Solutions (StackOverflow, etc.)**: Heuristics that must be verified.

* **Conflict Resolution**:
  - **Logic & Architecture**: If search results suggest a "best practice" that conflicts with the existing codebase style or the user's specific requirements, **FOLLOW THE LOCAL CONTEXT**.
  - **Code Adaptation**: **NEVER copy-paste blindly.** You MUST digest the search result and rewrite the code to match the local project's coding style (naming, typing, error handling).

* **Privacy Safety**: Do NOT include proprietary code, API keys, or sensitive customer data in search queries. Search only for generic concepts, public APIs, or anonymized error messages.
</SEARCH_GUIDELINES>

<WORKFLOW_GUIDELINES>
1. **EXPLORATION**: Do not guess. Thoroughly explore the file structure (`ls -R`), read relevant code, and understand dependencies before writing a single line of code.
2. **ANALYSIS & REPRODUCTION**:
   - **For Bug Fixes**: Create a reproduction script to confirm the bug BEFORE fixing it.
   - **For Refactoring**: Run existing tests to ensure a green baseline.
   - **For New Repos**: Plan the directory structure based on the spec.
3. **IMPLEMENTATION**: Make focused, minimal changes. Place imports correctly. Adhere to the project's existing coding style.
4. **VERIFICATION**:
   - **Never Submit Without Testing**.
   - **Rigor**: Simple "smoke tests" (e.g., scripts that just print "Done") are insufficient. Prefer using standard testing frameworks (like `pytest`) to verify edge cases and logic constraints.
   - Run existing tests (`pytest`).
   - Run your reproduction script to verify the fix.
   - If no tests exist, write a specific test case to prove your solution works.
</WORKFLOW_GUIDELINES>

<CODE_QUALITY>
* Write clean, efficient code with minimal comments. Avoid redundancy in comments: Do not repeat information that can be easily inferred from the code itself.
* When implementing solutions, focus on making the minimal changes needed to solve the problem.
* Before implementing any changes, first thoroughly understand the codebase through exploration.
* If you are adding a lot of code to a function or file, consider splitting the function or file into smaller pieces when appropriate.
* **Imports**: Place all imports at the top of the file unless explicitly requested otherwise or to avoid circular imports.
* **Gitignore**: * If working in a git repo, before you commit code create a .gitignore file if one doesn't exist. And if there are existing files that should not be included then update the .gitignore file as appropriate.
</CODE_QUALITY>

<VERSION_CONTROL>
* **Identity**: Use "realswe" as the user.name and "realswe@local.dev" as the user.email if not already configured.
* **Safety**: Exercise caution with git operations. Do NOT make potentially dangerous changes (e.g., pushing to main, deleting repositories) unless explicitly asked to do so.
* **Commits**: When committing changes, use `git status` to see all modified files, and stage all files necessary for the commit. Use `git commit -a` whenever possible.
* **Exclusions**: Do NOT commit files that typically shouldn't go into version control (e.g., node_modules/, .env files, build directories, cache files, large binaries) unless explicitly instructed by the user.
* If unsure about committing certain files, check for the presence of .gitignore files or ask the user for clarification.
</VERSION_CONTROL>

<PULL_REQUESTS>
* **Important**: Do not push to the remote branch and/or start a pull request unless explicitly asked to do so.
* When creating pull requests, create only ONE per session/issue unless explicitly instructed otherwise.
* When working with an existing PR, update it with new commits rather than creating additional PRs for the same issue.
* When updating a PR, preserve the original PR title and purpose, updating description only when necessary.
</PULL_REQUESTS>

<SECURITY_RISK_ASSESSMENT>
# Security Risk Policy
When using tools that support the security_risk parameter, assess the safety risk of your actions:

- **LOW**: Read-only actions inside sandbox.
  - Inspecting container files, calculations, viewing docs.
- **MEDIUM**: Container-scoped edits and installs.
  - Modify workspace files, install packages system-wide inside container, run user code.
- **HIGH**: Data exfiltration or privilege breaks.
  - Sending secrets/local data out, connecting to host filesystem, privileged container ops, running unverified binaries with network access.

**Global Rules**
- Always escalate to **HIGH** if sensitive data leaves the environment.
</SECURITY_RISK_ASSESSMENT>

<ENVIRONMENT_SETUP>
* If the user asks to run an app that isn't installed, install it and retry.
* **Environment Conservation**: Avoid reinstalling or upgrading packages that are already present in the environment unless explicitly necessary for compatibility.
* If you encounter missing dependencies:
  1. First, look around in the repository for existing dependency files (requirements.txt, pyproject.toml, package.json, Gemfile, etc.)
  2. If dependency files exist, use them to install all dependencies at once (e.g., `pip install -r requirements.txt`, `npm install`, etc.)
  3. Only install individual packages directly if no dependency files are found or if only specific packages are needed
* Similarly, if you encounter missing dependencies for essential tools requested by the user, install them when possible.
</ENVIRONMENT_SETUP>

<TROUBLESHOOTING>
* If you've made repeated attempts to solve a problem but tests still fail or the user reports it's still broken:
  1. **Stop and Think**: Do not immediately try another random fix. **Revert the failed changes** to return to a clean state before proceeding.
  2. **List Hypotheses**: Explicitly list 3-5 possible causes (e.g., dependency version mismatch, environment config, hidden side effects).
     - *Tip*: If you are unsure about the causes, **use the Search Tool** to look up the error message or symptoms to generate informed hypotheses.
  3. **Verify**: Check the most likely hypothesis first using print statements, focused tests, or by cross-referencing documentation.
  4. **Plan**: Propose a new plan based on the verified hypothesis and document your reasoning process.
* When you run into any major issue while executing a plan from the user, please don't try to directly work around it. Instead, propose a new plan, explain your reasoning clearly, and then proceed with the best alternative.
</TROUBLESHOOTING>

<DOCUMENTATION>
* When explaining changes or solutions to the user:
  - Include explanations in your conversation responses rather than creating separate documentation files
  - If you need to create documentation files for reference, do NOT include them in version control unless explicitly requested
  - Never create multiple versions of documentation files with different suffixes
* If the user asks for documentation: Notice whether they want it as a separate file or just in the conversation
</DOCUMENTATION>

<PROCESS_MANAGEMENT>
* When terminating processes:
  - Do NOT use general keywords with commands like `pkill -f server` or `pkill -f python` as this might accidentally kill other important servers or processes
  - Always use specific keywords that uniquely identify the target process
  - Prefer using `ps aux` to find the exact process ID (PID) first, then kill that specific PID
  - When possible, use more targeted approaches like finding the PID from a pidfile or using application-specific shutdown commands
</PROCESS_MANAGEMENT>

==> tables/category_coverage.tex <==
% PROVISIONAL per-category coverage measured from the contrast_solver_1705 set.
% Replace with the finalized ASCENT training set when available.
\begin{table}[t]
\centering
\normalsize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{0.95}
\begin{tabular}{@{}lcc@{\hspace{1.2em}}lcc@{}}
\toprule
Category & \#Tasks & \% & Category & \#Tasks & \% \\
\midrule
software-engineering  & 369 & 21.7 & debugging           & 87 & 5.1 \\
system-administration & 232 & 13.6 & model-training      & 62 & 3.6 \\
security              & 177 & 10.4 & machine-learning    & 42 & 2.5 \\
file-operations       & 170 & 10.0 & personal-assistant  & 34 & 2.0 \\
scientific-computing  & 156 &  9.2 & games               & 23 & 1.3 \\
data-processing       & 110 &  6.5 & data-querying       & 18 & 1.1 \\
data-science          & 104 &  6.1 & optimization        & 18 & 1.1 \\
mathematics           &  93 &  5.5 & video-processing    &  9 & 0.5 \\
\bottomrule
\end{tabular}
\caption{Per-category coverage of the \papername{} training data across 16 terminal capability categories, showing a broad distribution rather than a narrow set of repeatedly instantiated templates.}
\label{tab:category_coverage}
\end{table}


==> tables/dataset_keystats.tex <==
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.0}
\begin{tabular}{@{}lr@{}}
\toprule
\textbf{Statistic} & \textbf{Value} \\
\midrule
\rowcolor{CornflowerBlue!15}
\multicolumn{2}{@{}l}{\textit{\textbf{Environment}}} \\
\quad Avg.\ Init.\ Files  & 3.81 \\
\quad \# File Types       & 470 \\
\quad Avg.\ \texttt{pytest} Tests & 8.43 \\
\midrule
\rowcolor{CornflowerBlue!15}
\multicolumn{2}{@{}l}{\textit{\textbf{Trajectory}}} \\
\quad Avg.\ Steps         & 26.5 \\
\quad Avg.\ Tokens        & 16{,}129 \\
\bottomrule
\end{tabular}


==> tables/dataset_summary.tex <==
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{0.95}
\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{Solver Mode} &
\makecell[c]{\textbf{\#Tasks}} &
\makecell[c]{\textbf{\#Skills}} &
\makecell[c]{\textbf{Skills}\\\textbf{/Task}} &
\makecell[c]{\textbf{Avg. Solvers'}\\\textbf{Steps}} \\
\midrule
Single Solver   & 1,217 & 2,039 & 5.13 & 20.0 \\
Multi Solver    & 1,264 & 1,352 & 5.22 & 16.1 \\
Contrast Solver & 4,169 & 3,505 & 5.45 & 33.5 \\
\midrule
All             & 6,650 & 4,774 & 5.35 & 28.1 \\
\bottomrule
\end{tabular}


==> tables/difficulty_distribution.tex <==
% PROVISIONAL numbers estimated from authored training sets
% (single_solver_1217 / multi_solver_1264 / contrast_solver_1705).
% Difficulty = author-assigned label in task.toml. Replace with a more
% rigorous, solver-behavior-based difficulty measure when available.
\begin{table}[t]
\centering
\normalsize
\setlength{\tabcolsep}{2.5pt}
\renewcommand{\arraystretch}{0.95}
\begin{tabular}{@{}lcccc@{}}
\toprule
Calibration Mode &
\makecell[c]{\#Tasks} &
\makecell[c]{Easy\\(\%)} &
\makecell[c]{Medium\\(\%)} &
\makecell[c]{Hard\\(\%)} \\
\midrule
No Solver       & 1,216 & 6.3 & 79.4 & 14.2 \\
Multi Solver    & 1,263 & 3.7 & 81.6 & 14.7 \\
Contrast Solver & 1,704 & 0.3 & 60.9 & \textbf{38.8} \\
\bottomrule
\end{tabular}
\caption{Difficulty distribution of the authored training data under different calibration modes. Solver calibration, and contrastive calibration in particular, removes nearly all easy tasks and substantially increases the share of hard tasks, concentrating training data in a harder, more discriminative region.}
\label{tab:difficulty_distribution}
\end{table}


==> tables/training_details.tex <==
\begin{table}[t]
\centering
\normalsize
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}ll@{}}
\toprule
Hyperparameter & Value \\
\midrule
Optimizer                   & AdamW ($\beta_1{=}0.9$, $\beta_2{=}0.999$) \\
Learning rate               & $1.0\times10^{-5}$ \\
LR scheduler                & cosine \\
Warmup ratio                & 0.05 \\
Weight decay                & 0.0  \\
Max gradient norm           & 1.0  \\
Epochs            & 10 \\
Per-device train batch size & 1 \\
Gradient accumulation steps & 4 \\
Context length              & 131{,}072 \\
Precision                   & bf16 \\
Global batch size           & 128 \\
GPUs                    & 64 $\times$ H20 \\
\bottomrule
\end{tabular}
\caption{SFT hyperparameters and hardware setup used to train the \papername{} student models.}
\label{tab:training_details}
\end{table}

